Stylized Face Sketch Extraction via Generative Prior with Limited Data

Facial sketches are both a concise way of showing the identity of a person and a means to express artistic intention. While a few techniques have recently emerged that allow sketches to be extracted in different styles, they typically rely on a large amount of data that is difficult to obtain. Here, we propose StyleSketch, a method for extracting high-resolution stylized sketches from a face image. Using the rich semantics of the deep features from a pretrained StyleGAN, we are able to train a sketch generator with 16 pairs of face and the corresponding sketch images. The sketch generator utilizes part-based losses with two-stage learning for fast convergence during training for high-quality sketch extraction. Through a set of comparisons, we show that StyleSketch outperforms existing state-of-the-art sketch extraction methods and few-shot image adaptation methods for the task of extracting high-resolution abstract face sketches. We further demonstrate the versatility of StyleSketch by extending its use to other domains and explore the possibility of semantic editing. The project page can be found in https://kwanyun.github.io/stylesketch_project.

==> figures_tex/3_04_generator.tex <==
\begin{figure}[!htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=0.9\linewidth]{figures/generator.png}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %

  \caption{\label{fig:network}
           stylesketch generator.}
\end{figure}

==> figures_tex/5_05_training_figure.tex <==
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=0.9\linewidth]{figures/LPIPS_over_iterations.png}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %

  \caption{LPIPS over iterations with and without the initial stage.}
   \label{fig:training initial stage}
\end{figure}     

==> figures_tex/5_07_numdata.tex <==
\begin{figure}[!t]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=1\linewidth]{figures/numberofData.png}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %

  \caption{\label{fig:datasetablataion}
           \fixe{The number of training data pairs used and their corresponding model performance.}}
\end{figure}

==> figures_tex/5_08_generated.tex <==
\begin{figure*}[!htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=1\linewidth]{figures/ours_sketch.png}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %

  \caption{\label{fig:generated results}
           Results of our method in nine different styles, each trained with 16 data.}
\end{figure*}

==> tables/quant_comparison.tex <==

\begin{table*}[t]
\centering
\scriptsize % reduce font size
\setlength{\tabcolsep}{2pt} % reduce column spacing
\renewcommand{\arraystretch}{1.5} % increase row height
\caption{Quantitative results of comparison with baselines. The best LPIPS scorea are annotated in \textbf{bold} while the best FID scores are \underline{underlined}.} \vspace{-10pt}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cccccccccc|}
\noalign{\smallskip}\noalign{\smallskip}\hline

\hline
Sketch styles & SKSF-A(style 1) & SKSF-A(style 2) & SKSF-A(style 3) & SKSF-A(style 4) & SKSF-A(style 5) & SKSF-A(style 6) & SKSF-A(style 7)           & APDrawing           & CUFS                  & AVERAGE            \\ \hline
    Methods      & \multicolumn{10}{c|}{\textbf{LPIPS↓}/\underline{FID}↓}                                                     \\ \hline
    
\textit{Ours}                & \textbf{0.1669}/\underline{62.24} & 0.1552/90.12 & 0.1665/76.53 & \textbf{0.1405}/\underline{75.11} & 0.1956/175.68 & \textbf{0.1025}/86.54 & \textbf{0.1112}/149.01 & 0.2078/94.13 & 0.0513/91.54 & \textbf{0.1442}/100.10  \\ 
\hline 
RSSA with limited               & 0.2231/198.09 & 0.1876/168.23 & 0.2026/138.86 & 0.1789/129.10 & 0.2111/183.57 & 0.1615/122.60 & 0.1515/232.31 & 0.2531/133.87 & 0.1019/173.39 & 0.1868/164.44 \\
Few-shot with limited                & 0.2487/138.63 & 0.2389/157.19 & 0.2393/116.46 & 0.2125/116.49 & 0.2570/204.09 & 0.1854/114.73 & 0.1400/229.58 & 0.2697/154.13 & 0.0911/160.73 & 0.2092/154.67 \\
\hline
JoJoGAN with one                & 0.1946/141.32 & 0.1781/104.86 & 0.1957/116.84 & 0.1634/85.82 & 0.2078/177.44 &0.1188/107.34 & 0.1237/219.68 & 0.2239/114.42 & 0.0604/133.68 & 0.1629/133.48 \\
MTG with one               & 0.2150/212.81 & 0.1891/181.43 & 0.2048/154.94 & 0.1780/131.29 & 0.2072/246.72 & 0.1332/122.38 & 0.1401/231.39 & 0.2202/80.53 & 0.0591/134.41 & 0.1718/166.21 \\
\hline 
Learn-to-draw with limited                & 0.2212/260.91 & 0.2053/294.25 & 0.2218/311.29 & 0.1888/278.71 & 0.2217/353.55 & 0.1619/209.86 & 0.1436/277.72 & 0.2659/181.49 & 0.0577/78.36 & 0.1875/249.57 \\ 
APDrawing++ with limited                & 0.1945/125.09 & 0.1645/92.47 & 0.1782/116.77 & 0.1619/162.56 & 0.1838/189.84 & 0.1294/104.16 & 0.1220/182.46 & 0.2016/81.28 & 0.0518/82.62 & 0.1542/126.36 \\ 
\hline
Ref2sketch with full                & 0.1998/129.96 & 0.1595/\underline{56.85} & 0.1828/80.58 & 0.1597/81.45 & 0.1836/\underline{141.48} & 0.1345/\underline{73.98} & 0.1423/\underline{143.15} & 0.2547/82.27 & 0.0735/106.83 & 0.1656/99.62 \\ 
Learn-to-draw with full                & 0.2082/166.18 & 0.1795/127.41 & 0.1988/143.14 & 0.1753/161.79 & 0.2059/271.74 & 0.1520/162.97 & 0.1362/245.96 & 0.2685/145.70 & \textbf{0.0488}/\underline{71.46} & 0.1748/166.26 \\
APDrawing++ with full                & 0.1838/101.21 & \textbf{0.1529}/70.15 & \textbf{0.1646}/\underline{72.04} & 0.1543/85.34 & \textbf{0.1696}/157.11 & 0.1177/77.73 & 0.1141/153.64 & \textbf{0.1809}/\underline{62.41} & 0.0674/99.67 & 0.1450/\underline{97.70} \\

\hline 
\end{tabular}%}
\label{Tab:baseline}
\end{table*} 




==> tables/quant_comparison_new.tex <==
\begin{table*}[t]
\centering
\scriptsize % reduce font size
\setlength{\tabcolsep}{2pt} % reduce column spacing
\renewcommand{\arraystretch}{1.5} % increase row height
\caption{Quantitative results of comparison with baselines. The best LPIPS scores are annotated in \textbf{bold} while the best FID scores are \underline{underlined}.} \vspace{-10pt}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cccccccccc|}
\noalign{\smallskip}\noalign{\smallskip}

\hline
Sketch styles & SKSF-A(style 1) & SKSF-A(style 2) & SKSF-A(style 3) & SKSF-A(style 4) & SKSF-A(style 5) & SKSF-A(style 6) & SKSF-A(style 7)           & APDrawing           & CUFS                  & AVERAGE            \\ \hline
    Methods      & \multicolumn{10}{c|}{\textbf{LPIPS↓}/\underline{FID}↓}                                                     \\ \hline
    
\textit{Ours with limited(16)}                & \textbf{0.1669}/\underline{62.24} & 0.1552/90.12 & 0.1665/76.53 & \textbf{0.1405}/\underline{75.11} & 0.1956/175.68 & \textbf{0.1025}/86.54 & \textbf{0.1112}/149.01 & 0.2078/94.13 & 0.0513/91.54 & \textbf{0.1442}/100.10  \\ 
\hline 
RSSA with limited               & 0.2231/198.09 & 0.1876/168.23 & 0.2026/138.86 & 0.1789/129.10 & 0.2111/183.57 & 0.1615/122.60 & 0.1515/232.31 & 0.2531/133.87 & 0.1019/173.39 & 0.1868/164.44 \\
Few-shot with limited               & 0.2487/138.63 & 0.2389/157.19 & 0.2393/116.46 & 0.2125/116.49 & 0.2570/204.09 & 0.1854/114.73 & 0.1400/229.58 & 0.2697/154.13 & 0.0911/160.73 & 0.2092/154.67 \\
JoJoGAN with limited                & 0.1789/132.61 & 0.1611/125.93 & 0.1727/97.36 & 0.1466/87.30 & 0.1973/105.87 &0.1046/123.45 & 0.1176/188.08 & 0.2340/111.18 & 0.0588/138.46 & 0.1524/123.36 \\
MTG with limited             & 0.2166/233.77 & 0.1920/192.30 & 0.1966/174.30 & 0.1724/128.35 & 0.2311/141.06 & 0.1315/117.53 & 0.1356/205.67 & 0.2252/102.32 & 0.0708/127.37 & 0.1746/158.07 \\
Learn-to-draw with limited                & 0.2212/260.91 & 0.2053/294.25 & 0.2218/311.29 & 0.1888/278.71 & 0.2217/353.55 & 0.1619/209.86 & 0.1436/277.72 & 0.2659/181.49 & 0.0577/78.36 & 0.1875/249.57 \\ 
APDrawing++ with limited                & 0.1945/125.09 & 0.1645/92.47 & 0.1782/116.77 & 0.1619/162.56 & 0.1838/189.84 & 0.1294/104.16 & 0.1220/182.46 & 0.2016/81.28 & 0.0518/82.62 & 0.1542/126.36 \\ 
\hline
JoJoGAN with one                & 0.1946/141.32 & 0.1781/104.86 & 0.1957/116.84 & 0.1634/85.82 & 0.2078/177.44 &0.1188/107.34 & 0.1237/219.68 & 0.2239/114.42 & 0.0604/133.68 & 0.1629/133.48 \\
MTG with one               & 0.2150/212.81 & 0.1891/181.43 & 0.2048/154.94 & 0.1780/131.29 & 0.2072/246.72 & 0.1332/122.38 & 0.1401/231.39 & 0.2202/80.53 & 0.0591/134.41 & 0.1718/166.21 \\
\hline
Ours with four                & 0.1987/154.58 & 0.1733/202.58 & 0.1997/173.34 & 0.1534/118.85 & 0.2337/154.44 &0.1161/118.03 & 0.1226/193.49 & 0.2181/123.55 & 0.0532/106.85 & 0.1632/149.52 \\

JoJoGAN with four                & 0.1859/115.96 & 0.1711/119.76 & 0.1847/97.51 & 0.1586/91.11 & 0.2053/113.51 &0.1131/118.92 & 0.1206/196.41 & 0.2173/102.62 & 0.0585/128.90 & 0.1572/120.52 \\
MTG with four               & 0.2153/198.69 & 0.1916/192.98 & 0.2084/169.29 & 0.1722/130.97 & 0.2233/153.48 & 0.1260/112.76 & 0.1399/217.35 & 0.2393/98.55 & 0.0769/120.78 & 0.1770/154.98 \\
\hline
Ours with eight                & 0.1837/92.66 & 0.1596/121.56 & 0.1735/99.79 & 0.1551/85.09 & 0.2087/95.71 &0.1125/94.84 & 0.1180/193.59 & 0.2165/131.66 & 0.0541/106.34 & 0.1535/113.47 \\

JoJoGAN with eight                & 0.1793/129.59 & 0.1623/125.49 & 0.1771/95.85 & 0.1521/80.62 & 0.1981/100.46 &0.1085/115.88 & 0.1205/195.89 & 0.2152/105.99 & 0.0576/147.59 & 0.1523/121.93 \\
MTG with eight               & 0.2143/220.65 & 0.1916/200.23 & 0.2042/156.24 & 0.1801/138.63 & 0.2198/132.23 & 0.1208/101.97 & 0.1385/204.48 & 0.2283/96.75 & 0.0725/118.54 & 0.1745/152.19 \\
\hline
Ref2sketch with full                & 0.1998/129.96 & 0.1595/\underline{56.85} & 0.1828/80.58 & 0.1597/81.45 & 0.1836/\underline{141.48} & 0.1345/\underline{73.98} & 0.1423/\underline{143.15} & 0.2547/82.27 & 0.0735/106.83 & 0.1656/99.62 \\ 
Learn-to-draw with full                & 0.2082/166.18 & 0.1795/127.41 & 0.1988/143.14 & 0.1753/161.79 & 0.2059/271.74 & 0.1520/162.97 & 0.1362/245.96 & 0.2685/145.70 & \textbf{0.0488}/\underline{71.46} & 0.1748/166.26 \\
APDrawing++ with full                & 0.1838/101.21 & \textbf{0.1529}/70.15 & \textbf{0.1646}/\underline{72.04} & 0.1543/85.34 & \textbf{0.1696}/157.11 & 0.1177/77.73 & 0.1141/153.64 & \textbf{0.1809}/\underline{62.41} & 0.0674/99.67 & 0.1450/\underline{97.70} \\

\hline 
\end{tabular}%}
\label{Tab:baseline}
\end{table*} 


